VRS-NeRF: Visual Relocalization with Sparse Neural Radiance Field

Visual relocalization is a key technique to autonomous driving, robotics, and virtual/augmented reality. After decades of explorations, absolute pose regression (APR), scene coordinate regression (SCR), and hierarchical methods (HMs) have become the most popular frameworks. However, in spite of high efficiency, APRs and SCRs have limited accuracy especially in large-scale outdoor scenes; HMs are accurate but need to store a large number of 2D descriptors for matching, resulting in poor efficiency. In this paper, we propose an efficient and accurate framework, called VRS-NeRF, for visual relocalization with sparse neural radiance field. Precisely, we introduce an explicit geometric map (EGM) for 3D map representation and an implicit learning map (ILM) for sparse patches rendering. In this localization process, EGP provides priors of spare 2D points and ILM utilizes these sparse points to render patches with sparse NeRFs for matching. This allows us to discard a large number of 2D descriptors so as to reduce the map size. Moreover, rendering patches only for useful points rather than all pixels in the whole image reduces the rendering time significantly. This framework inherits the accuracy of HMs and discards their low efficiency. Experiments on 7Scenes, CambridgeLandmarks, and Aachen datasets show that our method gives much better accuracy than APRs and SCRs, and close performance to HMs but is much more efficient.

==> tables/table_12scenes.tex <==
\setlength{\tabcolsep}{3.pt}

\begin{table*}
	%\footnotesize
	%\tiny
	\scriptsize
	\centering
		\begin{tabular}{lccccccccccccc}
			\toprule
			Method & kitchen1 & living1 & bed & kitchen2 & living2 &luke & gates362 & gates381 & lounge & manolis & 5a & 5b & Average\\
			AS~\cite{as} & 100 & 100 & 100 & 99.1 & 100 & 100 & 100 & 100 & 99.7 & 100 & 98.8 & 99.5 & 99.8 \\
			HLoc~\cite{hfnet} & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 99.5 & 100\\ 
			%DSAC 
			DSAC*~\cite{dsac} & 100 & 99.8 & 100 & 100 & 100 & 100 & 100 & 99.5 & 100 & 98.6 & 99.4 & 100 & 99.8 \\ 
			%ACE~\cite{ace2023} & 
			SFD2+IMP~\cite{sfd22023,imp2023} &  100 & 100 & 100 & 99.6 & 100 & 99.8 & 100 & 100 & 99.7 & 100 & 96.4 & 100 \\
			SP+SG~\cite{superpoint,superglue} & 100 & 100 & 100 & 99.6 & 100 & 99.8 & 100 & 100 & 99.7 & 100 & 97.8 & 100 & \\  
			\midrule
			%Ours & 
			\bottomrule
		\end{tabular}
\caption{\textbf{Localization accuracy on the RobotCar-Seasons dataset.} The best results are highlighted.}
\label{exp:tab:12scenes}
\end{table*}

==> tables/table_7scenes_12scenes.tex <==
\setlength{\tabcolsep}{8.pt}

\begin{table}
	%\footnotesize
	%\tiny
	\scriptsize
	\centering
		\begin{tabular}{lcc}
			\toprule
			Method & 7Scenes & 12Scenes \\
			\toprule
			AS (SIFT)~\cite{as} & 98.5\% & 99.8\% \\ 
			SP+SG~\cite{superpoint,superglue} & 95.7\% & 100\% \\
			SFD2+IMP~\cite{sfd22023,imp2023} & 95.7\% & 99.7\%\\
			\midrule
			%DSAC &  \\
			DSAC* & 96.0\% & 99.6\% \\
			ACE~\cite{ace2023} & 97.1\% & 99.9\% \\
			\midrule
			Ours & 97.3\% & 97.8\% \\
			Ours(C) & 97.3\% & 97.8\% \\
			%Ours & 
			\bottomrule
		\end{tabular}
\caption{\textbf{Localization accuracy on 7Scenes~\cite{sevenscenes2013} and 12Scenes~\cite{twelvescenes2016} datasets.}}
\label{tab:7scenes}
\end{table}

==> tables/table_landmarks.tex <==
\setlength{\tabcolsep}{4.pt}

\begin{table}
	\footnotesize
	%\tiny
	%\scriptsize
	\centering
		\begin{tabular}{lcc}
			\toprule
			Dataset & \#Scenes & \#Landmarks \\
			\midrule
			7Scenes (S)~\cite{7scenes2013} & 7 & 112 \\
			12Scenes (T)~\cite{12scenes2016} & 12 & 192 \\
			CambridgeLandmarks (C)~\cite{posenet} & 5 & 160 \\
			Aachen (A)~\cite{aachen} & 1 & 512 \\
			%RobotCar (R)~\cite{robotcar} & 1 & 512 \\
			\midrule
			CAST~\cite{7scenes2013, 12scenes2016, aachen, posenet} & 25 & 976\\
			\bottomrule
		\end{tabular}
\caption{\textbf{Number of landmarks in different datasets.} For 7Scenes and 12Scenes datasets, we assign each scene in the datasets 16 landmarks and therefore obtain $112 = 7\times16$ and $192 = 12 \times 16$ landmarks, respectively. Each scene in CambridgeLandmarks dataset has 32 landmarks, so this dataset has $160 = 5 \times 32$. Aachen has only one scene and 512 landmarks. We additionally create a new larger dataset, called CAST, by combining all of these datasets together with 976 landmarks in total to test the ability of our model.}
\label{tab:landmarks}
\end{table}

==> tables/table_map_size.tex <==
\setlength{\tabcolsep}{4.pt}

\begin{table*}
	%\footnotesize
	%\tiny
	\scriptsize
	\centering
		\begin{tabular}{lccccccc}
			\toprule
			 Dataset & Method & \# Reference images & \#3D points (M) & Local Descriptor Size (G) & Global Descriptor Size (G) & 3D Map size (G) & Total Size (G) \\
			\midrule
			\multirow{4}{*}{S} & SP+SG~\cite{superpoint,superglue,netvlad} & 26,000 & 0.66 & 14.6 & 0.79 & 0.50 & 15.90 \\
			& SFD2+IMP~\cite{sfd22023,imp2023} & 26,000 & 0.44  & 5.78 & 0.79 & 0.39 & 6.96\\ 
			& DSAC~\cite{dsac*} & 0 & 0 & 0 & & 0.03 & 0.03 \\
			& ACE~\cite{ace2023} & 0 & 0 & 0 & 0 & 0.004 & 0.004 \\
			& Ours & 0 & 0.43 & 0 & 0 & 0.60 & 0.60 \\ 
			& Ours(C)& 0 & 0.05 & 0 & 0 & 0.03 & 0.03 \\ 
			\midrule
			
			\multirow{4}{*}{T} & SP+SG~\cite{superpoint,superglue,netvlad} & 16,989 & 0.84 & 11.62 & 0.52 &  0.43 & 12.57\\
			& SFD2+IMP~\cite{sfd22023,imp2023} & 16,989 & 0.59 & 4.45 & 0.52 & 0.33 & 5.30 \\ 
			& DSAC~\cite{dsac*} & 0 & 0 & 0 & & 0.03 & 0.03 \\
			& ACE~\cite{ace2023} & 0 & 0 & 0 & 0 & 0.004 & 0.004 \\
			& Ours & 0 & 0.55 & 0 & 0 & 0.59 & 0.59\\ 
			& Ours(C)& 0 & 0.15 & 0 & 0 & 0.08 & 0.08\\ 
			\midrule
			
			\multirow{4}{*}{C} & SP+SG~\cite{superpoint,superglue,netvlad} & 5,365 & 1.65 & 10.81 & 0.16 & 0.63 & 11.60 \\
			& SFD2+IMP~\cite{sfd22023,imp2023} & 5,365 & 1.55 & 5.31 & 0.16 & 0.63 & 6.1 \\ 
			& DSAC~\cite{dsac*} & 0 & 0 & 0 & & 0.14 & 0.14 \\
			& ACE~\cite{ace2023} & 0 & 0 & 0 & 0 & 0.02 & 0.02 \\
			
			& Ours & 0 & 1.12 & 0 & 0 & 1.17 & 1.17\\ 
			& Ours(C)& 0 & 0.4 & 0 & 0 & 0.22 & 0.22\\ 
			\midrule
			
			\multirow{4}{*}{A} & SP+SG~\cite{superpoint,superglue,netvlad} & 6,697 & 2.15 & 13.83 & 0.20 & 0.72 & 14.76 \\
			& SFD2+IMP~\cite{sfd22023,imp2023} & 6,697 & 2.21 & 7.21 & 0.2 & 0.8 & 8.17 \\ 
			& Ours & 0 &1.81 & 0 &  0 & 1.63 & 1.63\\ 
			& Ours(C)& 0 & 1.33 &  0 & 0 & 0.72 & 0.72 \\ 
			\midrule
			
			\multirow{4}{*}{CAST} & SP+SG~\cite{superpoint,superglue,netvlad} &  & & & & & \\
			& SFD2+IMP~\cite{sfd22023,imp2023} & & & & & &\\ 
			& Ours & 0 & & & & & \\ 
			& Ours(C) & 0 & & & & & \\ 
			
			\bottomrule
		\end{tabular}
\caption{\textbf{Map size.} We show the number of number of reference image (\#Ref. images), 3D points (\#3D points) and the local descriptor (desc.), global descriptor size, 3D map size and the total size at test time. The datasets include 7Scenes (S), 12Scenes (T), CambridgeLandmarks (C), Aachen (A) and CAST.}
\label{tab:map_size}
\end{table*}

==> tables/table_methods.tex <==
\setlength{\tabcolsep}{2.pt}

\begin{table}
	%\footnotesize
	%\small
	\scriptsize
	\centering
	\begin{tabular}{lcccc}
		\toprule
		Method &  memory efficiency & time efficiency & accuracy & large-scale\\
		\midrule 
		APRs~\cite{posenet,glnet,mapnet} & \cmark & \cmark & {\color{red}\xmark} & \cmark \\
		SCRs~\cite{dsac,dsac++,localinstance} & \cmark & \cmark & \cmark & {\color{red}\xmark} \\ 
		HMs~\cite{hfnet,lbr,as} & {\color{red}\xmark} & {\color{red}\xmark}& \cmark & \cmark\\
		\textbf{?} & \cmark & \cmark & \cmark & \cmark \\
		\bottomrule 
	\end{tabular}
\caption{\textbf{Comparisons of APRs, SCRs, and HMs.}  APRs are fast but inaccurate; SCRs work well in small scenes but fail to scale up in large-scale environments; HMs have high accuracy and adaptability while are not efficient.}
\label{tab:methods}
\end{table}

==> tables/table_recognition.tex <==
\setlength{\tabcolsep}{2.pt}

\begin{table}
	%\footnotesize
	%\tiny
	\scriptsize
	\centering
		\begin{tabular}{lcc|cc}
			\toprule
			Dataset & \#Scenes & \#Landmarks & \#Keypoints & Precision@1 \\
			& & & \multicolumn{2}{c}{day, night} \\
			\midrule
			7Scenes~\cite{sevenscenes2013} & 7 & 112 & 412.7, NA & 80.0\%, NA \\
			12Scenes~\cite{twelvescenes2016} & 12 & 192 & 435.3, NA & 95.0\%, NA \\
			CambridgeLandmarks~\cite{posenet} & 5 & 160 & 4087.8, NA & 87.6\%, NA \\
			Aachen~\cite{aachen} & 1 & 512 & 3192.2, 3262.7 & 69.8\%, 49.7\% \\
			\bottomrule
		\end{tabular}
\caption{\textbf{Recognition results.} We report the number of scenes (\#Scenes), landmarks (\#Landmarks) and the average number of keypoints (\#keypoints), the precision @ top 1 on 7Scenes\cite{sevenscenes2013}, 12Scenes~\cite{twelvescenes2016}, CambrigeLandmarks~\cite{posenet} and Aachen datasets~\cite{aachen}.}
\label{tab:recognition}
\end{table}

==> tables/table_time.tex <==
\setlength{\tabcolsep}{4.pt}

\begin{table}
	%\footnotesize
	%\tiny
	\scriptsize
	\centering
		\begin{tabular}{lccc}
			\toprule
			Group & Method & Input size & Time (ms) \\
			\midrule
			\multirow{3}{*}{Local Feature} & SP~\cite{superpoint} & $1024\times1024$ & 13.1 \\
			%& R2D2~\cite{r2d2} & $1024\times1024$ & 72.4 \\
			& SFD2~\cite{sfd22023} & $1024\times1024$ & 33.2 \\
			Global Feature & NetVLAD~\cite{netvlad} & $1024\times1024$ & 32.5 \\
			\multirow{4}{*}{Matcher} & SG~\cite{superglue} & 4k $\times$ 4k & 146.5 \\
			& SG~\cite{superglue} & 2k $\times$ 2k & 52.2 \\
			& IMP~\cite{imp2023} & 4k $\times$ 4k &  \\
			& IMP~\cite{imp2023} & 2k $\times$ 2k &  \\
			& Ours & 4k $\times$ 4k & 52.0 \\
			& Ours & 2k $\times$ 2k & 17.0 \\
			\midrule
			\midrule
			& SP+NV+SG~\cite{superpoint,netvlad,superglue} & $1024\times1024$, 2k & 97.8 \\
			& SP+NV+SG~\cite{superpoint,netvlad,superglue} & $1024\times1024$, 4k & 192.1 \\
			& Ours & $1024\times1024$, 2k & \\
			\bottomrule
		\end{tabular}
\caption{\textbf{Running time.}}
\label{tab:time}
\end{table}
